Optimal Competitive Auctions

We study the design of truthful auctions for selling identical items in unlimited supply (e.g., digital goods) to n unit demand buyers. This classic problem stands out from profit-maximizing auction design literature as it requires no probabilistic assumptions on buyers' valuations and employs the framework of competitive analysis. Our objective is to optimize the worst-case performance of an auction, measured by the ratio between a given benchmark and revenue generated by the auction. We establish a sufficient and necessary condition that characterizes competitive ratios for all monotone benchmarks. The characterization identifies the worst-case distribution of instances and reveals intrinsic relations between competitive ratios and benchmarks in the competitive analysis. With the characterization at hand, we show optimal competitive auctions for two natural benchmarks. The most well-studied benchmark $\mathcal{F}^{(2)}(\cdot)$ measures the envy-free optimal revenue where at least two buyers win. Goldberg et al. [13] showed a sequence of lower bounds on the competitive ratio for each number of buyers n. They conjectured that all these bounds are tight. We show that optimal competitive auctions match these bounds. Thus, we confirm the conjecture and settle a central open problem in the design of digital goods auctions. As one more application we examine another economically meaningful benchmark, which measures the optimal revenue across all limited-supply Vickrey auctions. We identify the optimal competitive ratios to be $(\frac{n}{n-1})^{n-1}-1$ for each number of buyers n, that is $e-1$ as $n$ approaches infinity.

==> notations.tex <==

\section{Notations}
\label{sec:prelim}

The summary of our conventions on the notation:
 \begin{itemize}
 \item Number of agents (bidders) $\nbidder$.
 \item Auction $\auction$.
 \item Individual bid $\bidi$, true value $\vali$.
 \item Generic indexes/conventions on notations
       \begin{itemize}
       \item bidders --- $i,j$.
			 \item Vectors are in boldface script, e.g.  $\vals=(\val_1,\dots,\val_\nbidder)$.
       \item $f_i(\vals)$ --- numerical indexes below, real values and vectors in parenthesis.
       \end{itemize}
 \item Vector $\vals$ without $i$-th coordinate $\valsmi$.
 \item Use $\dist$ to denote a distribution of bids
 \item Use $\dist^*$ to denote the revenue equivalent distribution on the domain $\vali\ge 1$.
 \item $\mathcal{A}$ denotes an auction.
 \item $\distM$ denotes the space of auctions.
 \item $\distMech$ denotes a distribution of truthful auctions.
 \item $\F^{(2)}(\vals)$ - benchmark at point $\vals$.
 \item $\proj_i S$ denotes the projections of the set $S$ along the $i$-th coordinate.
 \item LP
       \begin{itemize}
       \item function that we want to implement $f(\bids)$.
       \item finite discretized support of bids $\support$.
       \item $z_i(\vals)=z_i(\valsmi,\vali)$ --- probability to set price $\vali$ for agent $i$ when the rest bid $\valsmi$.
       \item $x_i(\vals)=\sum_{\pricei=1}^{\vali}\pricei\cdot
              z_i(\valsmi,\pricei)$
       \item $w(t)=
             \begin{cases}
               \frac{1}{t(t+1)}, & \quad t\in[1,N-1] \\
							 \frac{1}{t}, & \quad   t=N
						\end{cases}$,
			 \item $\weight(\bids)=\prod_{k=1}^{\nbidder}w(\bid_k)$,
			 \item $\weight(\bidsmi)=\prod\limits_{k\neq i}w(\bid_k)$.
       \item $g_i(\valsmi)$ --- total mass along direction $i$ at the point
              $\valsmi$ (initially it is $1$).
       \item dual variables $y(\vals)$, $y_i(\valsmi)$.			
       \item Projection of a set $S$ along $i$-th coordinate $S_{\text{-}i}$
       \end{itemize}
 \end{itemize}
%

%

